Charting EDA: Characterizing Interactive Visualization Use in Computational Notebooks with a Mixed-Methods Formalism

Interactive visualizations are powerful tools for Exploratory Data Analysis (EDA), but how do they affect the observations analysts make about their data? We conducted a qualitative experiment with 13 professional data scientists analyzing two datasets with Jupyter notebooks, collecting a rich dataset of interaction traces and think-aloud utterances. By qualitatively coding participant utterances, we introduce a formalism that describes EDA as a sequence of analysis states, where each state is comprised of either a representation an analyst constructs (e.g., the output of a data frame, an interactive visualization, etc.) or an observation the analyst makes (e.g., about missing data, the relationship between variables, etc.). By applying our formalism to our dataset, we identify that interactive visualizations, on average, lead to earlier and more complex insights about relationships between dataset attributes compared to static visualizations. Moreover, by calculating metrics such as revisit count and representational diversity, we uncover that some representations serve more as "planning aids" during EDA rather than tools strictly for hypothesis-answering. We show how these measures help identify other patterns of analysis behavior, such as the "80-20 rule", where a small subset of representations drove the majority of observations. Based on these findings, we offer design guidelines for interactive exploratory analysis tooling and reflect on future directions for studying the role that visualizations play in EDA.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/OLD-06-representations-and-usage.tex <==
\section{Characterizing Representations and Usage}
\label{RESULTS-rep-usage}

Guided by RQ2, this section examines the relationship between \foutput{Representations} and analyst \fobs{Observations}. We investigate patterns in representation usage (\S\ref{RESULTS-80-20}) and explore how certain representations contribute to analysis planning and navigation (\S\ref{sec:planning-aids}). We also analyze how the introduction of interactive elements influences the content of observations during EDA sessions (\S\ref{attribute-addition}). Finally, we examine the strategies employed by analysts who achieve broad coverage in their exploratory analyses (\S\ref{broad-exploration}). Through these investigations, we aim to provide a comprehensive understanding of how different representations, particularly interactive visualizations, shape the EDA process and influence analytical outcomes.

% \subsection{Beyond Expected Use: How Analysts Leverage Representations}
\subsection{Temporality, Diversity, and Velocity}
\label{representation-overview}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/results/representation_usage_and_type.png}
  \caption{Left: Representation creation over time. Right: Heatmap of the number of times different \fvis{Visualizations} were used to make an \fobs{Observation}, according to \fobs{UtteranceType}.}
  \label{fig:output_creation_and_use}
\end{figure}

Our participants constructed 1169 \foutput{Outputs} across all \fall{Sessions}, on averaging 44 different outputs per session. Arbitrary code execution execution was the most common output, followed by \fvis{Visualizations}. Temporal patterns emerged (Fig.~\ref{fig:output_creation_and_use}-left), with code cells used most frequently at the beginning and end of sessions, while visualizations dominated from about 15\% into the session onwards.

%Looking at when participants made these outputs (Fig.~\ref{fig:output_creation_and_use}-left) reveals interesting temporal patterns. 
%Code cells were used most frequently near the beginning and end of analysis sessions and often involved functions that checked the measure of central tendancy of attributes. Starting approximately 15\% of the way through their sessions, participants began to switch to favoring visualizations\,---\,these representations were then used to form the bulk of their subsequent observations.

Based on this data, we compute two metrics of representation construction: \fmetric{representationDiversity}, which is the number of \textit{unique} representations constructed in an analysis session; and, \fmetric{representationVelocity}, or the rate at which representations were constructed over course of an analysis session.
As Figure~\ref{fig:output_creation_and_use} shows, these metrics are moderately correlated (Pearson's $r= 0.47$); we discuss their role within analysis sessions in a subsequent section (\S~\ref{broad-exploration}). 

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/results/velocity-diversity.png}
  \caption{Scatterplot of computed representationDiversity and representationalVelocity for each analysis session.}
  \label{fig:repDiversity-and-velocity}
  \vspace{-2em}
\end{figure}


Examining the intersection of \fvis{ChartTypes} and \fobs{Observations} (Fig.~\ref{fig:output_creation_and_use}(right)) reveals expected and surprising usage patterns.
% 
For instance, unsurprisingly, scatterplots were most frequently used to make utterances about \fobs{Relationships} while profiler views helped participants make \fobs{Variable} utterances. 
However, as this heatmap shows, participants would frequently use charts beyond their intended purposes or in ways that break with best practice. For instance, only 42\% of observations with profiler views were \fobs{Variable} utterances.  Similarly, in contrast
to visualization theory and visualization recommender systems, which emphasize perceptual effectiveness, participant P9, a data science instructor, specifically created a representation she called a “spaghetti plot”— a line chart with 180 different series overplotted. Ahead of creating the chart she commented “It’s going to be a bad idea”, but persisted precisely because she wanted to ensure that the plot itself was ineffective,

%For instance, \fobs{Variable} utterances constituted only 42\% of observations made with profiler views\,---\,even though, ostensibly, this is the core purpose of a columnar distribution of data values.
%Similarly, in contrast to visualization theory and visualization recommender systems, which emphasize perceptual effectiveness, participant P9, a data science instructor, specifically created a representation she called a \textit{``spaghetti plot''}\,---\,a line chart with 180 different series overplotted.



\subsection{Hover Patterns and Observations}
\label{sec:hover-telemetry}

We can also connect \foutput{Representations} and \fobs{Observations} through \foutput{Telemetry} data, by calculating two metrics: \fmetric{hoverTime}, the total time an analyst spent hovering over a representation; and, \fmetric{revisitCount}, or the number of times an analyst hovered over a particular representation.

% Connecting \fobs{Observations} to the specific \foutput{Output} they were made with enables us to consider the ways in which patterns of \foutput{Telemetry} are linked to patterns in forming insights. These patterns are used to calculate metrics such as \fmetric{hoverTime} and \fmetric{revisitCount}. 

\subsubsection{The '80-20 Rule': Why Some Visualizations Matter More}
\label{RESULTS-80-20}
Our analysis reveals an 80-20 threshold in representation usage during EDA. The \textit{top 20\%} of most frequently hovered representations accounted for 79\% of total \fmetric{hoverTime} and 75\% of observations. Representations in the \textit{top 20\%} had hover durations of at least 30 seconds and averaged 2.8 observations each, indicating deep engagement. In contrast, the \textit{bottom 80\%} averaged just 0.2 observations per representation. Two key factors distinguish these groups: the ability to encode multiple attributes simultaneously and interactivity.

Representations displaying information about multiple
variables simultaneously (e.g., profilers, correlation heatmaps, pairplots) were more common in the \textit{top-20} (22\% vs 2\% in the \textit{bottom-80}). Analysts engaged with these \textit{all-attribute representations} through ``touring'' behaviors (\S~\ref{RESULTS-Sequential-transitions}), systematically exploring different variable combinations every 5--15 seconds. These representations commanded longer average \fmetric{hoverTime} (67--169 seconds) compared to \foutput{Code Cells} used for quick statistical checks. Notably, \foutput{Code Cells} decreased from 48\% of the \textit{bottom-80} to just 9\% of the \textit{top-20}, averaging only 4.9 seconds of hovering per representation. 
% This contrast highlights the deeper engagement fostered by all-attribute representations during EDA.

%All attribute representations also had longer average hover times for these visualizations (67-169 seconds) when compared with \texttt{Code Cells} used for quick statistical checks (from 48\% of the \textit{bottom-80} to 9\% of \textit{top-20}, averaging 4.9 seconds of hovering per representation). 


%Representations displaying information about multiple variables simultaneously (e.g., profilers, correlation heatmaps, pairplots) were more common within the \textit{top-20}. These \textit{all-attribute representations} made up only 2\% of the \textit{bottom-80} but constituted 22\% of the \textit{top-20}, an 11X increase. Analysts engaged with these visualizations through the ``touring'' behaviors we previously described in \S~\ref{RESULTS-Sequential-transitions}, systematically exploring them and commenting on different variable combinations approximately every 5-15 seconds. This is underlined by the longest average hover times observed for all-attribute visualizations (67 seconds for profiles, 75 seconds for heatmaps, and 169 seconds for pairplots). Similarly, we see a marked decrease in \fmetric{hoverTime} 

Interactive visualizations were also more prevalent within the \textit{top-20} (24\% of the \textit{top-20} vs. 16\% of the \textit{bottom-80}). Analysts particularly favored the \texttt{highlight\_brush} as it enabled cross-linking data subsets across multiple charts. This technique was used in over 56\% of interactive representations in the \textit{top-20}, compared to 37\% in the \textit{bottom-80}
% , suggesting participant intuition for cross highlighting to explore relationships between variables. 
In contrast, \texttt{filter\_brush} and \texttt{pan\_zoom} interactions were less popular in frequently used visualizations, likely due to context loss and usability issues respectively.

%the \texttt{filter\_brush} technique, which filters out all non-selected data marks from view, was used in 30\% of the interactive scatterplots found within the \textit{bottom-80}. However, \texttt{filter\_brush} went to 2\% in the \textit{top-20}, a likely side effect of filtering obscuring important context in standalone charts. 

%Finally, \texttt{pan\_zoom} interactions, was the second most popular interaction technique in \textit{bottom-80} – present in over 31\% of interactive representations. However, declined to just 18\% in the \textit{top-20}. Analysts consistently struggled to find effective use for pan-zoom interactions, suggesting a lack of intuition for how this technique could enhance their analysis workflows. Out of the 16 instances in which pan-zoom was used, we observed only one instance where it successfully uncovered an insight that would have been difficult to obtain otherwise. In this case, participant P10 zoomed into a dense, overplotted region of a scatterplot to gain more resolution, and was able to reveal a pattern in the depicted data. However, even this success story was marred by discomfort\,---\,P10 added pan-zoom to a set of horizontally arranged scatterplots that shared a common y-axis; thus, the coordinated scrolling of all scatterplots made him feel disoriented, prompting him to request \textit{``can we turn that off?''}

% The general ineffectiveness of pan-zoom is surprising, given its prevalence as a default interaction in many interactive Python data visualization libraries (e.g. panzoom is the default behavior of Altair's \verb|[chart].interactive()| method). While pan-zoom interactions can be beneficial when thoughtfully designed\cite{schwab_evaluating_2019}, our study indicates that analysts may lack the necessary tools or mental models to leverage them successfully for typical statistical charts. This finding highlights a potential area for improvement in visualization libraries, prompting further investigation into how pan-zoom interactions could be redesigned or supplemented to better support EDA tasks.


% \subsubsection{Revisit Count: All-attribute visualizations that function as planning aids}
\subsubsection{All-Attribute Visualizations Aid Planning}
\label{sec:planning-aids}
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/results/scatterplot-planning-revisit.png}
  \caption{Average \fmetric{revisitCount} and count of \texttt{Plan of Action} utterances by \foutput{Representation}. Representations are colored by whether or not it is an \textit{all-attribute representation}. Representations to the left are typically one-off question-answering tools whereas representations to the right are frequently revisited when deciding analysis paths. %From least revisited to most: \foutput{Code Cell}, \foutput{Column Printouts}, \fvis{Stripplot}, \fvis{Lineplot}, \fvis{Scatterplot}, \fvis{Custom Dashboard}, \fvis{Histogram}, \fvis{Barplot}, \foutput{Table}, \foutput{Describe}, \fvis{Heatmap}, \fvis{Pairplot}, \fvis{Profile}, \foutput{Info}.
  }
  \vspace{-1em}
  \label{fig:revisiting-count}
\end{figure}


% A \foutput{Output's} \fmetric{revisitCount} is the number times a representation is revisited, revealing patterns of how analysts return to representations throughout their analysis process. 
As Figure~\ref{fig:revisiting-count} shows, high \fmetric{revisitCounts} (over 10 times) indicate that a representation serves as an process planning tool, aiding analysts in orienting themselves and preparing their next actions. For example, participant P5 created a correlation heatmap to identify the most strongly correlated attributes within her dataset. She frequently returned to this visualization, using it as a guide for selecting specific attributes to investigate further: \textit{``let's look at the one that is most positively correlated, which seems to be log GDP per capita. So I'll start with that variable''}. This led her to generate scatterplots and custom dashboards for deeper exploration. This approach proved effective, leading to 23 observations. 
Such action-planning is not restricted to only visual all-attribute representations\,---\,participants frequently revisited data frame outputs (including \texttt{df.describe}, \texttt{df.info}, and simply the tabular preview output) to formulate their plans.
% However, even with its minimal information scent, other All Attribute Representations like data tables still supported these type of planning behaviors. For example, when using \foutput{dataframe} printouts of the data table, participants often read individual record values and then formulate plans to analyze their data. 
For instance, P11 read through the individual values of a dataframe printout, commenting: \textit{``Of course, we cannot say for the whole thing [based on just the shown rows]. So my strategy will be like going through each of the variable here, and do the summary statistic.''} 
Looking across all \fobs{Observations} tuples in our dataset, all-attribute representations are associated with \texttt{Plan of Action} utterances at a rate of 5x more than other representations.


%Other examples included P6's who used a profiler to investigate the distributions of her data, finishing her univariate tour commenting \textit{"nothing looks especially interesting. So I guess this just means make a bunch of plots."}  




% \subsection{Attribute Addition: Interactive Visualizations Shift Analyst Behavior Towards Complex Data Relationships}
\subsection{An Interactive Draw Towards Complexity}
\label{attribute-addition}

When using interactive visualizations, we observed shifts in the types and number of attributes that analysts considered. An \textit{attribute addition} behavior appears prominently in analysts who are progressively exploring data relationships of escalating complexity, moving utterances from univariate distributions to bivariate relationships, and further morphing into multivariate analyses. For example, in the static condition participant P5 used the profiler visualization to analyze the univariate distributions of her columns, making 6 utterances about their distributions. At the beginning of the interactive session, she created an interactive version of the profiler visualization, and immediately began using it to analyze relationships\,---\,brushing on the chart to examine a target population and generating 6 new utterances about that population's relationship to variables. This pattern of behavior persisted across datasets for other participants (Fig.~\ref{fig:attribute-addition}~(left)).

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/results/horizontal-attribute-addition.png}
  \caption{Left: Numbers of Utterances between static and interactive versions of the profiler and scatterplot visualizations. The most common interaction techniques used for these representations were cross-filter brushes, tooltips, and filtering sliders. Right: Comparison of which data types were discussed in utterances in static vs. interactive visualizations. The plot indicates that there is a steep rise in multivariate relationship utterances in interactive visualizations}
  \label{fig:attribute-addition}
\end{figure}

% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[width=\textwidth]{figures/results/attribute-addition.png}
%   \caption{Left: Numbers of Utterances between static and interactive versions of the profiler and scatterplot visualizations. The most common interaction techniques used for these representations were a cross-filter brush, tooltips, and filtering sliders. Right: Differences in the data types discussed in utterances, split by whether or not a chart is interactive. The plot indicates that there is a steep rise in the amount of multivariate and continuous x continuous relationship utterances in the case of interactive visualizations}
%   \label{fig:attribute-addition}
% \end{figure*}


Filtering interactions in scatterplots also prompted shifts in behavior (Fig.~\ref{fig:attribute-addition}~(right)). While static scatterplots led to discussions of bivariate relationships, interactive versions prompted focus on multivariate relationships. to extract subsets from data clusters and pursued analysis paths to differentiate that cluster from the rest of the data. Another case of this was the use of the \texttt{filter\_slider}, an interaction technique which filters the chart to only the data value present in a particular value on a slider query widget. The shift we observe between these interactive and static charts presents the allure of interactive representations, seemingly pulling analysts towards investigating more complicated relationships even when those interactions are not actively being used. 

%Prior to the interactive session, we observed participants discussing bivariate relationships using scatterplots; however, when interaction was added, their utterances tended to focus on the multivariate relationships. Multiple participants used brushes to extract subsets from data clusters and pursued analysis paths to differentiate that cluster from the rest of the data. Another case of this was the use of the \texttt{filter\_slider}, an interaction technique which filters the chart to only the data value present in a particular value on a slider query widget. The shift we observe between these interactive and static charts presents the allure of interactive representations, seemingly pulling analysts towards investigating more complicated relationships even when those interactions are not actively being used. 
% While some investigations require considering multi-variate relationships,  tooling should be careful about making filter-based interactions available by default as their inclusion may alter the way in which analysts engage with their data. 

This attribute addition behavior varied across data types, with interactive visualizations primarily used for multivariate and continuous x continuous bivariate relationships. However, we note these patterns were most evident at the aggregate level, with individual participant data showing sparsity across data types. %Such descriptions warrant additional investigations to understand the role that interaction may play in drawing analyst hypotheses

% However, attribute addition behavior was not observed equally across data types. On average, our participants used interactive visualizations for multivariate (often all continuous variables) and continuous x continuous bivariate relationships (Fig.~\ref{fig:attribute-addition}~(right)). However we note the overall patterns are most salient at the aggregate level and the participant level contains sparsity in the utterances made for each participant for a given data type. Thus while we chose to report the results to fully describe the behavior that we saw, such descriptions warrant additional investigations to understand the role that interaction may play in drawing analyst hypotheses towards more multivariate and complex relationships and if such patterns exist over longer periods of time.

\subsection{Patterns of Broad Analysis Space Exploration}
\label{broad-exploration}

Previous studies of EDA offered characterization of analysis sessions based on the number of attributes analysts reasoned about~\cite{battle_characterizing_2019, wongsuphasawat_voyager_2017}. 
We extend this type of analysis, applying it to our definition of 
% define analysis states as the unique sets of attributes that are considered by an analyst during EDA. We extend this analysis through using our definition of
\fall{State} which encompasses the \foutput{Representations} analysts constructed, and how \freprusage{RepresentationUsage} affects \fobs{Observations} analysts made.
% \textbf{\fobs{Observations}} which combines attributes with \fobs{UtteranceType}
% \fobs{attributes} along with the \fobs{UtteranceType} which describes what is being said about the attributes. 
Follow Battle et al.'s method~\cite{battle_characterizing_2019}, we created binary histograms that represent whether or not our participants made a particular observation (e.g. observed the relationship between \textit{happiness} and  \textit{GDP}).  
Using the total count of observations made by our participants, we can compute for each participant what percent of total states visited, allowing us to rank our participants by the breadth of exploration. For example, participant P9, a data science instructor, made the most extensive \fobs{Dataset} observations across both static and interactive conditions (Fig.~\ref{fig:broad-states}~(1)). These observations occurred as P9 began each of her analysis sessions with a variable metadata tour: systematically going through each attribute in the data dictionary, spending time discussing what the variable meant and her opinions on its usefulness. 
Similarly, we observe the 5 participants who made the most \fobs{Variable} utterances (Fig.~\ref{fig:broad-states}~(2)) did so in the static condition using profile visualizations.
% , commenting on each variable's \fobs{distribution} through a distributional touring behavior. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/results/broad-analysis-states.png}
  \caption{Stripplot of \% of total unique \fobs{Observations} visited per analysis session, broken down by high level type and colored by Analysis Condition (Interactive or Static). 
  }
  \vspace{-1em}
  \label{fig:broad-states}
\end{figure}


In contrast, approaches for exploring a broad set of \fobs{Relationship} observations (Fig.~\ref{fig:broad-states}~(3)) reveals a diverse set of strategies. To investigate these patterns of exploration, we created attribute co-occurance heatmaps (Fig.~\ref{fig:teaser}) to ``fingerprint''  and explain these strategies: 
% \fall{Session} and provide illustrative case studies of how participant search behavior was structured by Representation-Usage and revealed through \foutput{Telemetry}.

\textbf{P8: Parameterized Search.} Driven by a clear goal and an aversion to \textit{``mindless''} exploration, P8 adopted a systematic, iterative approach reminiscent of a parameterized search through \foutput{Representations} and \fvis{Encodings}. She explored the analysis space by cycling through which attributes were mapped to encodings (e.g., \texttt{scatterplot(y=happiness, x=column[index])}), methodically investigating potential relationships between each attribute and the outcome variable. When she encountered specific patterns of interest, she then modified her scatterplot, adding interactions such as brushes and tooltips to investigate outliers and subsets. The resultant fingerprint visualization depicts a focused analysis centered around the outcome variable, with some targeted off-diagonal probes into the country, investigated using tooltips and brushes.  %Other similar analyses: 92ghd48xe, 3r2sh20ei.

% \textbf{P3: Iterative Deepening.} P3's approach was guided by emergent patterns in the data, resembling an iterative deepening search that is commonly used in graph traversal and game-playing algorithms.
% He generated scatterplots based on his intuition about interesting variable relationships, largely ignoring the outcome variable at the outset. This is reflected in his focus on predictor variables, evident in his thumbprint visualization. Upon noticing clusters within a plot, he investigated  their characteristics, iterating through both interaction and encodings (adding tooltips, brushes and \fvis{color} encodings) to identify potential explanatory variables. This behavior is captured in his high \fmetric{representationalVelocity} and \fmetric{representationDiversity} (each the highest out of all 26 analyses as shown in \ref{fig:repDiversity-and-velocity}), suggesting he wasn't wedded to a single visualization type but rather explored various options to gain deeper insights. This iterative deepening process ultimately led to a scattered thumbprint reflecting his serendipitous journey through attribute space, driven by unexpected findings. 

\textbf{P3: Iterative Deepening.} P3's approach resembled an iterative deepening search, guided by emergent patterns. He generated scatterplots based on intuition, focusing on predictor variables rather than the outcome. Upon noticing clusters, he iteratively added \fvis{Interaction} and \fvis{Encodings} to explore further. This approach led to the highest \fmetric{representationalVelocity} and \fmetric{representationDiversity} (Fig.~\ref{fig:repDiversity-and-velocity}), reflecting a flexible, serendipitous exploration.

%Other similar analyses: 4728juiz, s92hoei, E1D39056, 8v892iige.

\textbf{P6: Heuristic-Guided Best First Search.} P6's approach mirrored a best-first search algorithm, combining methodical planning with opportunistic exploration. She began with a cross-filtered \fvis{Profile} for bivariate exploration, then pivoted to a correlation \fvis{Heatmap} as her guiding heuristic. This heatmap became her analytical compass, revisiting it 35 times throughout her session. When a promising variable emerged, P6 seamlessly transitioned to a custom interactive dashboard, leveraging a \fvis{Scatterplot}, \fvis{Profile}, and \fvis{Countplot} for deeper, multivariate analysis. This strategic interplay between broad correlation assessment and focused multivariate investigation produced a cohesive analysis. P6's thumbprint visualization reveals a targeted exploration of direct predictors along the bottom row, complemented by thoughtful off-diagonal probes into potential confounders. Her approach exemplifies how a well-chosen heuristic can guide an efficient yet comprehensive exploration of complex data spaces.

%\textbf{P6: Heuristic-Guided Best First Search.} P6 combined a methodical foundation with a responsive, opportunistic approach characteristic of best-first search \cite{pearl1984heuristics}. This approach prioritizes exploring the most promising nodes (observation-analysis states) within a search space based on a pre-defined heuristic. P6's analysis mirrored this approach. Her initial bivariate exploration using a cross-filtered \fvis{profile} set the stage for a more targeted investigation guided by a \fvis{correlation heatmap}. She guided her search through the correlation of attributes with her outcome variable, revisiting the correlation matrix 35 times during her analysis showcasing a high \fmetric{revisitCount}. After locating a variable to investigate she would conduct a multivariate analysis using a custom interactive dashboard (made of a \fvis{scatterplot}, \fvis{profile}, and \fvis{countplot}). This approach is reflected in her high revisit count, which captured the number of times she revisited the correlation matrix. This strategy produced a cohesive analysis that investigated both direct predictors and potential confounders of the outcome variable, as evidenced by her targeted analysis along the bottom row and off-diagonal considerations in her thumbprint visualization. %Other similar Analyses: iurmer28. 


% \subsection{Thinking in the Language of Interaction: Reasoning about Interface Rules to Form Hypotheses}
\subsection{Thinking in the Language of Interaction}
\label{RESULT:language-of-interaction}
In interaction design, perceived affordances \cite{norman_design_2013} signal the operations a user believes are possible within an interface. Well-designed affordances establish interaction dynamics\,---\,the rules governing how users interact with the interface. Our study revealed that data scientists reasoned about these dynamics to generate new analytical hypotheses. In other words, they translated ``the language of interaction'' into novel analytical questions.
% 
As participant P8 described: \textit{``My thought of intersecting High GDP and High Life-Expectancy [countries] happened precisely because there was interaction... I was thinking, 'Oh I wonder if multi-select works'... That is actually what led me to think, 'Oh this would also be interesting on an analytical level.'''}. Later she commented that such an insight \textit{``would not have occurred to me if not for the fact I was working with an interactive visualization.''} 

% Participant P6's insights emerged from a similar process of experimentation.  Having successfully used ALX's copy-and-paste technique to paste filters between charts, he began to consider the broader possibilities this interaction technique offered for filtering his current visualization. While browsing other charts, he stumbled upon a bar plot showing the count of records over time. Intrigued, he initially tested if the copy-and-paste mechanic would function in this context. However, a spark ignited: rather than a simple test of function, he realized it would be more insightful to filter on the most recent years of data. This act of guided experimentation, prompted by the affordances of the interaction design (rather than performing the interaction itself and observing any updates), led him to discover an unexpected trend in life expectancy over time.

Participant P6 demonstrated a similar process of experimentation. While exploring the copy-and-paste filtering technique, he realized its potential for analyzing recent years' data in a time-series bar plot. This guided experimentation, prompted by the interaction design's affordances rather than the interaction itself, led to an unexpected discovery about life expectancy trends.

These observations suggest that interactive features play a more generative role in analysis than typically acknowledged. While literature often emphasizes interactions as task-completion tools, our findings indicate that affordances can actively shape analytical thinking. This insight has implications for both interaction design and future studies of interaction in data analysis. Designers should consider how to reify interaction dynamics to promote analytical reasoning, while researchers should investigate how different interaction cues influence not just usage \cite{boy_suggested_2016}, but also how analysts conceptualize potential analyses. 


